Center-of-mass energy determination using $e^+e^-$ to $\mu^+\mu^-$ $(\gamma)$ events at future $e^+e^-$ colliders

Methods for measuring the absolute center-of-mass energy, $\sqrt{s}$, and its distribution, are investigated for future $e^+e^-$ Higgs-factory colliders using in situ $e^+e^-$ collisions. We emphasize the potential of an estimator based on the measurement of muon momenta that we denote $\sqrt{s}_p$. It can be determined with high precision in $e^+e^-$ to $\mu^+\mu^-$($\gamma$) events while being sensitive to effects from beam energy spread, beamstrahlung, initial-state radiation (ISR), final-state radiation (FSR), crossing angle, and detector resolution. The measurement precision is enabled by a high-precision low-mass tracker; the reported performance estimates are based on full simulation of the tracker response of the ILD detector concept for the ILC operating at $\sqrt{s} = 250$ GeV. The underlying statistical precision is 1.9 ppm for a 2.0 ab$^{-1}$ dataset at ILC. The ultimate utility will depend largely on how well one can calibrate and maintain the tracker momentum scale.

==> ChangeLog.tex <==
\section{Change Log}
\begin{enumerate}
\item Add change log to track changes with respect to 2209.03281v1.
\item Added line numbers to facilitate commenting.
\item Changed x to E in Appendix B. Some minor 
rephrasing in App. B.
\item Included second talk title in T. Barklow reference.
\item multiline eqn B.1
\item reduce number of ``some''s in L362-L365 (Outlook)
%\item Fig10 added: $\sqrtsp$ (gen. level) (same as Fig 8) but with fit range 
%identical to Figs 4 and 9. Will keep only Fig 8 or Fig 10.
\item Fig 10 added (cheats $M_{3}$).
\item Resized 3-body and triangles diagram (Fig 6).
\item Description of Fig 10 in the text.
\item Added explanation to Appendix A of the quadratic solution.
\item Boldface 3-vector notation throughout.
\item Moved sa,ca,ta shorthand to first mention.
\item Made mods that were quick to implement suggested by Brendon.
\item Added siunitx package for typographical appearance of eg. microns around line 93.
\item Added consolidated event table and discussion.
\item Addressed Alberto's comments.
\item Added crossing-angle diagram.
\item Updated event table.
\item Added clickable URLs to most references.
\item Added unpolarized estimate
\item Added explicit momentum scale prospects
\item Updated momentum resolution 
number to 0.14\% from 0.17\%.
\end{enumerate}

\begin{enumerate}
\item Add change log to track changes with respect to 2209.03281v2.
\item Correct formula in footnote 1 re synchrotron radiation beam energy spread 
and add new reference.
\item Minor wording changes in intro and fix minor typos in outlook.
\end{enumerate}

==> EventTable.tex <==

\section{Draft Event Tables}

\begin{table}[hbt]
\begin{center}
\begin{tabular}{|c|r|}
\hline
   Variable                 &   Value [GeV]        \\  \hline 
     $\Ebm$                 &   114.55             \\  
     $\Ebp$                 &   124.64             \\ 
     $\Ediff$               &    -5.04             \\     
     $\sqrt{s}$             &   238.97             \\ 
     $M_{12}$               &   238.97             \\
     $p_{12}$               &    10.22             \\        
     $M_{3}$                &     0.00             \\
     $\sqrtsp$              &   249.26             \\ 
     $\sqrtsp$ (true $\Ediff$)     &   238.97      \\    \hline
\end{tabular}
\end{center}
\caption{Event 36}
\label{tab-example0}
\end{table}

\begin{table}[hbt]
\begin{center}
\begin{tabular}{|c|r|}
\hline
   Variable                 &   Value [GeV]        \\  \hline 
     $\Ebm$                 &   125.32             \\  
     $\Ebp$                 &   121.08             \\ 
     $\Ediff$               &     2.12             \\     
     $\sqrt{s}$             &   246.35             \\ 
     $M_{12}$               &    94.62             \\
     $p_{12}$               &   104.74             \\     
     $M_{3}$                &    31.27             \\
    $\sqrtsp$              &   245.88              \\   %C2
    $\sqrtsp$ (true $\Ediff$)   &   241.60         \\     %C3
    $\sqrtsp$ (true $M_{3}$)    &   250.45         \\     %C4
    $\sqrtsp$ (true $\Ediff$ \& $M_{3}$)    &   246.35      \\   \hline %C5
\end{tabular}
\end{center}
\caption{Event 58}
\label{tab-example0}
\end{table}
% Looks like there is a small inconsistency between true sqrt(s) and 
% fully cheated?

\begin{table}[hbt]
\begin{center}
\begin{tabular}{|c|r|}
\hline
   Variable                 &   Value [GeV]        \\  \hline 
     $\Ebm$                 &   124.87             \\  
     $\Ebp$                 &   124.49             \\ 
     $\Ediff$               &     0.19             \\     
     $\sqrt{s}$             &   249.35             \\ 
     $M_{12}$               &   249.30             \\
     $p_{12}$               &     1.73             \\
     $M_{3}$                &     0.00             \\
    $\sqrtsp$               &   249.65              \\     %C2
    $\sqrtsp$ (true $\Ediff$)   &   249.35         \\     %C3
    $\sqrtsp$ (true $M_{3}$)    &   249.65         \\     %C4
    $\sqrtsp$ (true $\Ediff$ \& $M_{3}$)    &   249.35      \\   \hline %C5
\end{tabular}
\end{center}
\caption{Event 63}
\label{tab-example0}
\end{table}

\begin{table}[hbt]
\begin{center}
\begin{tabular}{|c|r|}
\hline
   Variable                 &   Value [GeV]        \\  \hline 
     $\Ebm$                 &   124.75             \\  
     $\Ebp$                 &   116.24             \\ 
     $\Ediff$               &     4.26             \\     
     $\sqrt{s}$             &   240.84             \\ 
     $M_{12}$               &    82.34             \\
     $p_{12}$               &   101.66             \\
     $p_{12}^{z}$           &   $-101.65$          \\     
     $M_{3}$                &     0.55             \\
     $\sqrtsp$              &   232.47             \\ 
     $\sqrtsp$ (true $\Ediff$)     &   240.84             \\    \hline
\end{tabular}
\end{center}
\caption{Event 69}
\label{tab-example1}
\end{table}


\begin{table}[hbt]
\begin{center}
\begin{tabular}{|c|r|}
\hline
   Variable                 &   Value [GeV]        \\  \hline 
     $\Ebm$                 &   122.77             \\  
     $\Ebp$                 &   110.12             \\ 
     $\Ediff$               &     6.33             \\     
     $\sqrt{s}$             &   232.53             \\ 
     $M_{12}$               &    92.26             \\
     $p_{12}$               &   105.43             \\
     $p_{12}^{z}$           &   $+105.43$          \\
     $M_{3}$                &     0.00             \\
     $\sqrtsp$              &   245.53             \\ 
     $\sqrtsp$ (true $\Ediff$)         &   232.53             \\    \hline
\end{tabular}
\end{center}
\caption{Event 88}
\label{tab-example2}
\end{table}

==> OldResultsTable.tex <==
%\begin{block}{Statistical uncertainties in ppm on $\sqrt{s}$ for $\mumu$ channel}
\begin{table}[hbt]
\begin{center}
\begin{tabular}{|r|c|c|r|r|r|}
\hline
$L_\mathrm{int}$ [ab$^{-1}$] & Poln [\%] & Gold & Silver & Bronze & All categories  \\ \hline
0.9  &  $-80,+30$ & 6.5 & 3.1 & 8.5 & 2.7\\
0.9  &  $+80,-30$ & 7.7 & 3.4 & 9.6 & 3.0\\
0.1  &  $-80,-30$ & 26   & 12.1  & 33 & 10.4 \\
0.1  &  $+80,+30$ & 29   & 13.0  & 41 & 11.4\\  \hline
2.0  &  Combined  & 4.8  & 2.2 & 6.2 & {\bf 1.9} \\ \hline
\end{tabular}
\end{center}
\caption{
Fractional errors on the mean parameter, $\mu$, of the Gaussian peak component 
when fitting with the 5-parameter Crystal Ball function with 
all 4 shape parameters fixed to their best-fit values.}
\label{tab:results}
\end{table}

==> ToDoList.tex <==
\section{To do list and topics under investigation for potential inclusion}
\begin{enumerate}
%\item Include $M_3$ cheated generator level distribution.
%\item Table with examples. Can coalesce several events into one table. See current 
%draft tables in Appendix E.
%\item Can we show that the general formula 
%amounts also to E12* + p12* but after boosting 
%using the correct x and z boost components??
%\item Add coordinates system diagram.
\item Optimize figure size.
%\item Be more explicit on tracker momentum scale prospects.
\item Be more explicit 
on ILD tracker momentum resolution?
\item Be more explicit on center-of-mass energy 
precision goals re physics targets.
\item Maybe replace Fig 7 with the center-of-mass energy estimator??
%\item Add clickable URLs to references?
\item Add ILD logos to plots with ILD simulated data.
\item Include residuals plots.
\item Add apples-to-apples estimate for angles method comparison.
\item Obtain center-of-mass energy dependence of the estimate.
%\item Give unpolarized precision estimate too.
\item Explore making more quality bins for better precision.
\item Explore what is going on with the discrepant region?? Given that Fig 9 works very well, it must be some artefact/feature of the technique.
\item Improve RooFit displays of parameters??
\item Use correct boost and see effect of just 
detector resolution.
\item We should also try running 
the IDR-S detector model 
(B=4.0T but smaller radius).
\item Add more details on generator radiation model?
%\item REMOVE LINE NUMBERS!
%\item Double-check that all links are clickable
\end{enumerate}

==> mybib-backup.tex <==
%THIS IS NOW A BACKUP - make changes 
% to the clickable version.
\begin{thebibliography}{99}

%\cite{Roser:2022sht}
\bibitem{Roser}
T.~Roser \textit{et al.}
``Report of the Snowmass 2021 Collider Implementation Task Force,''
[arXiv:2208.06030 [physics.acc-ph]].
%0 citations counted in INSPIRE as of 31 Aug 2022

%\cite{Bagger:2022zyy}
\bibitem{Bagger}
J.~A.~Bagger \textit{et al.}
``Higgs Factory Considerations,''
[arXiv:2203.06164 [hep-ex]].
%0 citations counted in INSPIRE as of 31 Aug 2022

%\cite{ALEPH:2005ab}
\bibitem{LEP1}
S.~Schael \textit{et al.} [ALEPH, DELPHI, L3, OPAL, SLD, LEP Electroweak Working Group, SLD Electroweak Group and SLD Heavy Flavour Group],
``Precision electroweak measurements on the $Z$ resonance,''
Phys. Rept. \textbf{427}, 257-454 (2006)
doi:10.1016/j.physrep.2005.12.006
[arXiv:hep-ex/0509008].
%2818 citations counted in INSPIRE as of 06 Sep 2022

%\cite{Anashin:2015rca}
\bibitem{Anashin:2015rca}
V.~V.~Anashin \textit{et al.}
``Final analysis of KEDR data on J/\ensuremath{\psi} and \ensuremath{\psi}(2S) masses,''
Phys. Lett. B \textbf{749}, 50-56 (2015)
doi:10.1016/j.physletb.2015.07.057
%24 citations counted in INSPIRE as of 01 Sep 2022
 
%\cite{Blondel:2019jmp}
\bibitem{Blondel:2019jmp}
A.~Blondel \textit{et al.}
``Polarization and Centre-of-mass Energy Calibration at FCC-ee,''
[arXiv:1909.12245 [physics.acc-ph]].
%18 citations counted in INSPIRE as of 22 Aug 2021

%\cite{Wilson:2016hne}
\bibitem{Wilson:2016hne}
G.~W.~Wilson,
``Updated Study of a Precision Measurement of the W Mass from a Threshold Scan Using Polarized $\rm{e}^-$ and $\rm{e}^+$ at ILC,''
[arXiv:1603.06016 [hep-ex]].

%\cite{Seidel:2013sqa}
\bibitem{Seidel:2013sqa}
K.~Seidel, F.~Simon, M.~Tesar and S.~Poss,
``Top quark mass measurements at and above threshold at CLIC,''
Eur. Phys. J. C \textbf{73}, no.8, 2530 (2013)
doi:10.1140/epjc/s10052-013-2530-7
[arXiv:1303.3758 [hep-ex]].
%133 citations counted in INSPIRE as of 03 Sep 2022

%\cite{Yokoya:2019rhx}
\bibitem{Yokoya:2019rhx}
K.~Yokoya, K.~Kubo and T.~Okugi,
``Operation of ILC250 at the Z-pole,''
[arXiv:1908.08212 [physics.acc-ph]].
%9 citations counted in INSPIRE as of 05 Sep 2022

\bibitem{GWWMPI}
G.W.~Wilson, 
``Measuring the luminosity weighted average centre-of-mass energy with radiative $\mathrm{Z}^{0}$ events'', Talk presented in the ECFA/DESY Workshop on Physics 
and Detectors for a Linear Collider, MPI Munich, September 1996.

%\cite{Brinkmann:1997ws}
\bibitem{Brinkmann:1997ws}
R.~Brinkmann, G.~Materlik, J.~Rossbach and A.~Wagner,
``Conceptual design of a 500-GeV $\ee$ linear collider with integrated X-ray laser facility. Vol. 1-2,''
DESY-97-048.
%98 citations counted in INSPIRE as of 03 Sep 2022

%\cite{ALEPH:2006cdc}
\bibitem{ALEPH:2006cdc}
S.~Schael \textit{et al.} [ALEPH Collab.],
``Measurement of the W boson mass and width in $\ee$ collisions at LEP,''
Eur. Phys. J. C \textbf{47}, 309-335 (2006)
doi:10.1140/epjc/s2006-02576-8
[arXiv:hep-ex/0605011].
%74 citations counted in INSPIRE as of 01 Sep 2022

%\cite{OPAL:2004xxz}
\bibitem{OPAL:2004xxz}
G.~Abbiendi \textit{et al.} [OPAL Collab.],
``Determination of the LEP beam energy using radiative fermion-pair events,''
Phys. Lett. B \textbf{604}, 31-47 (2004)
doi:10.1016/j.physletb.2004.10.046
[arXiv:hep-ex/0408130].
%17 citations counted in INSPIRE as of 01 Sep 2022

%\cite{L3:2003vcr}
\bibitem{L3:2003vcr}
P.~Achard \textit{et al.} [L3 Collab.],
``Measurement of the Z boson mass using $\ee \to \mathrm{Z} \gamma$ events at center of mass energies above the Z pole,''
Phys. Lett. B \textbf{585}, 42-52 (2004)
doi:10.1016/j.physletb.2004.01.074
[arXiv:hep-ex/0402001].
%16 citations counted in INSPIRE as of 01 Sep 2022

%\cite{DELPHI:2006ymr}
\bibitem{DELPHI:2006ymr}
J.~Abdallah \textit{et al.} [DELPHI Collab.],
``A determination of the centre-of-mass energy at LEP2 using radiative 2-fermion events,''
Eur. Phys. J. C \textbf{46}, 295-305 (2006)
doi:10.1140/epjc/s2006-02506-x
[arXiv:hep-ex/0602016].
%11 citations counted in INSPIRE as of 01 Sep 2022

%\cite{Hinze:2005kh}
\bibitem{Hinze:2005kh}
A.~Hinze and K.~Monig,
``Measuring the beam energy with radiative return events,''
eConf \textbf{C050318}, 1109 (2005)
[arXiv:physics/0506115].
%10 citations counted in INSPIRE as of 04 Sep 2022

%\cite{Hinze:2005xt}
\bibitem{Hinze:2005xt}
A.~Hinze,
``Determination of beam energy at TESLA using radiative return events,''
LC-PHSM-2005-001.
%0 citations counted in INSPIRE as of 04 Sep 2022

\bibitem{Barklow}
T.~Barklow, 
``Physics Impact of Detector Performance'' 
and ``Measurement of the Beam Energy and Lumi Spectrum Using Mu Pairs'', 
Talks presented in the 2005 International Linear Collider Workshop (LCWS05), Stanford, March 2005.

\bibitem{GWW-LC2013}
G.W.~Wilson, 
``Investigating in-situ $\sqrt{s}$ determination with $\mumu(\gamma)$'', 
Talk presented in the European Linear Collider Workshop (ECFA, LC2013), 
Hamburg, May 2013.

%\cite{Wilson:2020arh}
\bibitem{Wilson:2020arh}
G.W.~Wilson [ILD concept group],
``Precision Electroweak Measurements with ILC250,''
PoS \textbf{ICHEP2020}, 347 (2021)
doi:10.22323/1.390.0347
%1 citations counted in INSPIRE as of 03 Sep 2022

%\cite{ILCInternationalDevelopmentTeam:2022izu}
\bibitem{ILCInternationalDevelopmentTeam:2022izu}
A.~Aryshev \textit{et al.} [ILC International Development Team],
``The International Linear Collider: Report to Snowmass 2021,''
[arXiv:2203.07622 [physics.acc-ph]].
%35 citations counted in INSPIRE as of 05 Sep 2022

%\cite{ILDConceptGroup:2020sfq}
\bibitem{ILDConceptGroup:2020sfq}
H.~Abramowicz \textit{et al.} [ILD Concept Group],
``International Large Detector: Interim Design Report,''
[arXiv:2003.01116 [physics.ins-det]].
%67 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Yokoya:1991qz}
\bibitem{Yokoya:1991qz}
K.~Yokoya and P.~Chen,
``Beam-beam phenomena in linear colliders,''
Lect. Notes Phys. \textbf{400}, 415-445 (1992)
doi:10.1007/3-540-55250-2\_37
%84 citations counted in INSPIRE as of 03 Sep 2022

%\cite{Poss:2013oea}
\bibitem{Poss:2013oea}
S.~Poss and A.~Sailer,
``Luminosity Spectrum Reconstruction at Linear Colliders,''
Eur. Phys. J. C \textbf{74}, no.4, 2833 (2014)
doi:10.1140/epjc/s10052-014-2833-3
[arXiv:1309.0372 [physics.ins-det]].
%29 citations counted in INSPIRE as of 03 Sep 2022

%\cite{Bambade:2019fyw}
\bibitem{Bambade:2019fyw}
P.~Bambade \textit{et al.}
``The International Linear Collider: A Global Project,''
[arXiv:1903.01629 [hep-ex]].
%222 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Kilian:2007gr}
\bibitem{Kilian:2007gr}
W.~Kilian, T.~Ohl and J.~Reuter,
``WHIZARD: Simulating Multi-Particle Processes at LHC and ILC,''
Eur. Phys. J. C \textbf{71}, 1742 (2011)
doi:10.1140/epjc/s10052-011-1742-y
[arXiv:0708.4233 [hep-ph]].
%793 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Moretti:2001zz}
\bibitem{Moretti:2001zz}
M.~Moretti, T.~Ohl and J.~Reuter,
``O'Mega: An Optimizing matrix element generator,''
[arXiv:hep-ph/0102195 [hep-ph]].
%446 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Schulte:1997nga}
\bibitem{Schulte:1997nga}
D.~Schulte,
``Study of Electromagnetic and Hadronic Background in the Interaction Region of the TESLA Collider,''
DESY-TESLA-97-08.
%43 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Ohl:1996fi}
\bibitem{Ohl:1996fi}
T.~Ohl,
``CIRCE version 1.0: Beam spectra for simulating linear collider physics,''
Comput. Phys. Commun. \textbf{101}, 269-288 (1997)
doi:10.1016/S0010-4655(96)00167-1
[arXiv:hep-ph/9607454].
%142 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Jadach:2022mbe}
\bibitem{Jadach:2022mbe}
S.~Jadach, B.~F.~L.~Ward, Z.~Was, S.~A.~Yost and A.~Siodmok,
``Multi-photon Monte Carlo event generator KKMCee for lepton and quark pair production in lepton colliders,''
[arXiv:2204.11949 [hep-ph]].
%0 citations counted in INSPIRE as of 06 Sep 2022

\bibitem{LCWS21}
G.W.~Wilson, 
``High Precision Tracker Momentum-Scale Calibration with Particle Decays at ILC'',
Talk presented in the 2021 International Linear 
Collider Workshop (LCWS21), Europe (virtual), March 2021.

%\cite{Rodriguez:2020qhf}
\bibitem{Rod2020}
P.~B.~Rodr\'\i{}guez 
\textit{et al.}
``Calibration of the momentum scale of a particle physics detector using the Armenteros-Podolanski plot,''
JINST \textbf{16}, no.06, P06036 (2021)
doi:10.1088/1748-0221/16/06/P06036
[arXiv:2012.03620 [physics.ins-det]].
%0 citations counted in INSPIRE as of 31 Aug 2022

\bibitem{AP-paper}
 J. Podolanski and R. Armenteros (1954), \emph{III. Analysis of V-events}, 
 The London, Edinburgh, and Dublin Philosophical Magazine and Journal of Science, 45:360, 13-30, 
 %DOI: 10.1080/14786440108520416 

%\cite{Verkerke:2003ir}
\bibitem{Verkerke:2003ir}
W.~Verkerke and D.~P.~Kirkby,
``The RooFit toolkit for data modeling,''
eConf \textbf{C0303241}, MOLT007 (2003)
[arXiv:physics/0306116].
%849 citations counted in INSPIRE as of 06 Sep 2022

%\cite{Cheng:2016ykr}
\bibitem{Cheng:2016ykr}
J.~H.~Cheng \textit{et al.}
``Determination of the total absorption peak in an electromagnetic calorimeter,''
Nucl. Instrum. Meth. A \textbf{827}, 165-170 (2016)
doi:10.1016/j.nima.2016.05.010
[arXiv:1603.04433 [physics.ins-det]].
%16 citations counted in INSPIRE as of 05 Sep 2022

%12 citations counted in INSPIRE as of 03 Sep 2022

%\cite{Wilson:2016tto}
%\bibitem{Wilson:2016tto}
%G.~W.~Wilson,
%``Precision Electroweak Measurements at a Future $e^+e^-$ Linear Collider,''
%PoS \textbf{ICHEP2016}, 688 (2016)
%doi:10.22323/1.282.0688
%2 citations counted in INSPIRE as of 03 Sep 2022



%Also include a top scan paper.

\end{thebibliography}
